A Solver-Free Framework for Scalable Learning in Neural ILP Architectures

There is a recent focus on designing architectures that have an Integer Linear Programming (ILP) layer within a neural model (referred to as Neural ILP in this paper). Neural ILP architectures are suitable for pure reasoning tasks that require data-driven constraint learning or for tasks requiring both perception (neural) and reasoning (ILP). A recent SOTA approach for end-to-end training of Neural ILP explicitly defines gradients through the ILP black box (Paulus et al. 2021) - this trains extremely slowly, owing to a call to the underlying ILP solver for every training data point in a minibatch. In response, we present an alternative training strategy that is solver-free, i.e., does not call the ILP solver at all at training time. Neural ILP has a set of trainable hyperplanes (for cost and constraints in ILP), together representing a polyhedron. Our key idea is that the training loss should impose that the final polyhedron separates the positives (all constraints satisfied) from the negatives (at least one violated constraint or a suboptimal cost value), via a soft-margin formulation. While positive example(s) are provided as part of the training data, we devise novel techniques for generating negative samples. Our solution is flexible enough to handle equality as well as inequality constraints. Experiments on several problems, both perceptual as well as symbolic, which require learning the constraints of an ILP, show that our approach has superior performance and scales much better compared to purely neural baselines and other state-of-the-art models that require solver-based training. In particular, we are able to obtain excellent performance in 9 x 9 symbolic and visual sudoku, to which the other Neural ILP solver is not able to scale.

==> sections/exp_keypoint_matching_yatin.tex <==
\subsection{Keypoint matching}
Here we experiment on a real world task of matching key points between two images of different objects of same type. 
The input $\inp$ consists of a pair of images $(I_1,I_2)$ of same type, \eg, cats, along with a shuffled list of coordinates of $k$ keypoints, \eg, tail, nose \etc, in both images. 
The task is to match the same keypoints in the two images with each other.
The ground truth constraint enforces a bijection between the keypoints in the two images.
For matching $k$ keypoints, the output $\outp$ is represented as a $k \times k$ binary permutation matrix, \ie, entries in a row or column should sum to $1$.

With the constraints known, \citet{rolinek&al20b} recently proposed a SOTA model that differentiates through a specialized graph-matching solver using the technique proposed in \cite{vlastelica&al20}.
Like \cite{paulus&al21}, our objective is not to compete against the SOTA method, but demonstrate that our method can also learn the constraints along with the backbone model parameterizing the cost vector.

\begin{wraptable}{r}{0.4\linewidth}
\vspace*{-2.5ex}
\caption{\small Number of train and test samples for datasets with different keypoints}
\vspace{-1.5ex}
\label{tab:keypointdata}
\resizebox{\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}l|rrrr@{}}
\toprule
\textbf{Num Keypoints} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{5}} & \multicolumn{1}{c}{\textbf{6}} & \multicolumn{1}{c}{\textbf{7}} \\ \midrule
\textbf{\#Test} & 10,474 & 9,308 & 7,910 & 6,580 \\
\textbf{\#Train} & 43,916 & 37,790 & 31,782 & 26,312 \\ \bottomrule
\end{tabular}
}
\vspace*{-1.5ex}
\end{wraptable}
\textbf{Dataset details:}
We experiment with image pairs in SPair-17k \cite{} dataset that has been used for the task of keypoint matching in the SOTA paper \cite{rolinek&al20b}.
Note that the learnt ILP in a neural ILP model works with a fixed dimension of output variables and thus we can't create a common model for image pairs with different number of matched keypoints, even though the backbone architecture parameterizing the cost is the same (handling this is a direction for future work).
Thus, we artificially create 4 datasets for 4,5,6 and 7 keypoints. %Notice that dataset for $k$ keypoints include all image pairs with more than $k$ pairs annotated. 
While training and testing models for $k$ keypoints, we randomly sample any $k$ annotated pairs from input image pairs that have more than $k$ keypoints annotated. See \cref{tab:keypointdata}.



\textbf{Baselines:}
Here we compare against a strong neural baseline which is same as the backbone model parameterizing the $k^2$ dimensional cost vector in \cite{rolinek&al20b}.
We denote the parameters of this backbone as $\theta_\cost$.
A feature vector for each keypoint in an image is first obtained by passing the image through a pre-trained VGGNet \cite{}.
These feature vectors are then used to initialize the node embeddings of a Graph with a node corresponding to a keypoint in an image.
Final node embedding obtained after a few steps of message passing in the graph is used as the final feature vector for each keypoint.
The cost $\cost_{ij}$ for matching keypoint $i$ in one image with keypoint $j$ in the other image is nothing but the negative of dot product similarity between the two feature vectors.
In the neural baseline, oblivion to the underlying constraints, we simply match $i^{th}$ keypoint in image 1 with $\argmin_j \cost_{i,j}$.
Training is done by minimizing the Binary Cross Entropy loss between the ground truth $\gtruth_{ij}$ and $\sigma(-\cost_{ij})$ where $\sigma$ is the sigmoid function. 
During testing of the neural model, in addition to the greedy matching as above, we also run a constrained inference with ground truth constraints and learnt cost (`Neural + CI' in \cref{tab:keypoint}. Note that the constraints are not used while training of the neural baseline.

In addition to $\theta_\cost$, we also learn the constraint matrix $\A$ and $\rhs$ in our model.

\textbf{Training details:
}
For each $k$, we train a separate Neural ILP model with $2k$ learnable constraints: same as the number of ground truth constraints.
In our method, for keypoints 5,6 and 7, we initialize the backbone cost parameters $\theta_\cost$ with the one obtained by training it on 4 keypoints.
\ycom{We start with a temprature $\tau=0.5$ and anneal it by a factor of $0.2$ at $10^{th}$ and $30^{th}$ epoch.
}

\begin{wraptable}{r}{0.5\linewidth}
\vspace*{-2.5ex}
\caption{\small Pointwise accuracy for matching keypoints in two images. Neural+CI is the ILP inference with the known constraints over the cost learnt by neural model.}
\vspace{-1.5ex}
\label{tab:keypoint}
\resizebox{\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}lrrrr@{}}
\toprule
 %& \multicolumn{4}{c}{\textbf{\% accuracy}} \\ %\midrule
\multicolumn{1}{l|}{\textbf{Num Keypoints}} & \multicolumn{1}{c|}{\textbf{4}} & \multicolumn{1}{c|}{\textbf{5}} & \multicolumn{1}{c|}{\textbf{6}} & \multicolumn{1}{c}{\textbf{7}} \\ \midrule
\multicolumn{1}{l|}{\textbf{Neural}} & \multicolumn{1}{r|}{81.98\%} & \multicolumn{1}{r|}{78.93\%} & \multicolumn{1}{r|}{76.06\%} & 74.68\% \\
\multicolumn{1}{l|}{\textbf{Neural+CI}} & \multicolumn{1}{r|}{83.32\%} & \multicolumn{1}{r|}{80.28\%} & \multicolumn{1}{r|}{77.68\%} & 76.66\% \\
\multicolumn{1}{l|}{\textbf{CombOptNet}} & \multicolumn{1}{r|}{\textbf{83.63\%}} & \multicolumn{1}{r|}{80.91\%} & \multicolumn{1}{r|}{77.29\%} & 76.28\% \\
\multicolumn{1}{l|}{\textbf{Ours}} & \multicolumn{1}{r|}{83.50\%} & \multicolumn{1}{r|}{\textbf{80.98\%}} & \multicolumn{1}{r|}{\textbf{78.62\%}} & \textbf{76.80\%} \\ \bottomrule
\end{tabular}
}
\vspace*{-1.5ex}
\end{wraptable}
\textbf{Results and discussion:}
\Cref{tab:keypoint} presents the percentage of keypoints matched correctly by different models. 
Both CombOptNet and our method achieve similar performance.
Note that we obtain a gain of ~2 points over the purely neural baseline without the knowledge of constraints.
This is almost same as the gain obtained by constrained inference with known constraints on top of neural model.
For this task, we did not observe any gain in the training time over CombOptNet. This is expected as the bottleneck here is the backbone neural model parameterizing the cost function.
Even though our method spends less time in each iteration, it takes more number of iterations to train, balancing out the gain by speeding up each iteration.



==> sections/exp_random_constraints_yatin.tex <==
\subsection{Random constraints}
\textbf{Task description:}
These are synthetic experiments borrowed from \citeauthor{paulus&al21}.
The training data $\traindata = \{(\cost_s, \gtruth_s) | s \in \integerrange{1}{S}\}$ is created by first generating a random polyhedron $\polyhedron \subseteq \outspace$ by sampling $m'$ hyperplanes $\{\constraint{\arow{i}'}{\rhs'_i} \ | \ \arow{i}', \rhs'_i \in \mathbb{R}^n, i \in \integerrange{1}{m'}\}$ in an $n$ dimensional bounded continuous space $\outspace$. A cost vector $\cost_s \in \mathbb{R}^n$ is then randomly sampled and corresponding $\gtruth_s$ is obtained as  $\gtruth_s = \argmin_{\var \in \polyhedron} \cost_s^T\var, \var \in \mathbb{Z}^n$.

Given a dataset $\traindata$, our objective is to learn a constraint matrix $\A$ and vector $\rhs$ such that for a ground truth $(\cost, \gtruth)$ pair, 
$\gtruth = \argmin_{\var \in \outspace} \cost^T\var$,   $\var \in \mathbb{Z}^n$, and $\A\var + \rhs \ge \zerovector$.

\begin{table}[]
%\begin{wraptable}{r}{0.8\linewidth}
\small
\captionof{table}{\small Mean $\pm$ std err of the vector accuracy ($\model_\Theta(\inp) = \gtruth$) and training time over the 5 datasets. Number of learnable constraints is twice the number of ground truth constraints.}
\label{tab:randomconstraints}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}lcrrrrrrr@{}}
\toprule
 & \multicolumn{8}{c}{\textbf{Vector Accuracy}} \\ \midrule
 & \multicolumn{4}{c}{\textbf{Binary}} & \multicolumn{4}{c}{\textbf{Dense}} \\
\textbf{} & \textbf{1} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{2}} & \multicolumn{1}{c}{\textbf{4}} & \multicolumn{1}{c}{\textbf{8}} \\
\textbf{CombOptNet} & \multicolumn{1}{r}{100  $\pm$ 5} & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 \\
\textbf{Ours} & \multicolumn{1}{r}{100  $\pm$ 5} & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 \\
 & \multicolumn{8}{c}{\textbf{Training Time}} \\
\textbf{CombOptNet} & \multicolumn{1}{r}{100  $\pm$ 5} & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 \\
\textbf{Ours} & \multicolumn{1}{r}{100  $\pm$ 5} & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 & 100  $\pm$ 5 \\ \bottomrule
\end{tabular}
}
\end{table}
%\end{wraptable}
%\textbf{Dataset details}: \\
\textbf{Dataset details:}
Restricting $\outspace$ to $[0,1]^n$ and $[-5,5]^n$ results in two variations which \citeauthor{paulus&al21} call \textbf{`binary datasets'} and \textbf{`dense datasets'} respectively.
For both of them, we experiment with four different settings in $n=16$ dimensional space by varying the number of ground truth constraints as $m'=1,2,4,$ and $8$.
For each $m'$, we train a separate Neural ILP model for the first 5 out of the 10 datasets provided by \citeauthor{paulus&al21} and report mean over the 5 models.
The training data in each case consists of $1600$ $(\cost,\outp)$ pairs and model performance is tested for $1000$ cost vectors.

\textbf{Hyperparameters and training details} are exactly the same as for sudoku, except for number of learnable constraints. Here, we keep number of learnable constraints as twice the number of ground truth constraints, \ie, $m= 2m'$. 
This is because it achieves the best performance for the baseline CombOptNet as reported in \citeauthor{paulus&al21}.

\textbf{Results and discussion:}
\ycom{TODO after the table gets filled.}
%\begin{table}[]


==> sections/exp_sudoku_yatin.tex <==
\subsection{Symbolic and visual sudoku}

\textbf{Task description:}
\begin{comment}
\begin{gather*}
\gtruth = \argmin \cost^T\var \ \  \text{\ \ subject to} \\ 
\sum\limits_{i=1}^{k} \var_{i,j,l} = 1 \forall j,l \in \integerrange{1}{k} ; 
\sum\limits_{j=1}^{k} \var_{i,j,l} = 1 \forall i,l \in \integerrange{1}{k} ; 
\sum\limits_{l=1}^{k} \var_{i,j,l} = 1 \forall i,j \in \integerrange{1}{k} ; \\
\sum\limits_{i=i'}^{i'+ \sqrt{k}}
\sum\limits_{j=j'}^{j'+ \sqrt{k}} \var_{i,j,l} = 1 \forall i',j' \in \integerrange{1}{\sqrt{k}}, 
l \in \integerrange{1}{k}
\end{gather*}
\end{comment}
This task involves learning the rules of the sudoku puzzle.
A $k \times k$ sudoku puzzle 
can be viewed as an ILP with $4k^2$ equality constraints over $k^3$ binary variables \cite{bartlett&al08}.
The $k^3$ dimensional binary input vector $\inp$ and the corresponding solution $\gtruth$ are created by representing each of the $k^2$ cells of the puzzle by a $k$ dimensional binary vector which takes a value of $1$ at $i^{th}$ dimension if and only if the cell is filled by digit $i$. 
Empty cells in the input are represented by a $k$ dimensional zero vector $\zerovector$.
In the case of symbolic sudoku, the cost vector is nothing but negative of the input $\inp$, \ie, 
$\cost = -\inp$.
Our objective is to learn the constraint matrix $\A = \fnA(\inp; \theta_\A) = \theta_\A$ and vector $\rhs = \fnrhs(\inp; \theta_\rhs) = \theta_\rhs$, representing the linear constraints of sudoku.

For \textbf{visual sudoku}, the input $\inp$ is an image of a sudoku puzzle where a digit is randomly replaced by one of its image in MNIST dataset \cite{}.
Unlike symbolic sudoku, the cost vector must be inferred from the input image.
To do so, we use a CNN based neural network, LeNet \cite{} to first decode each of the $k^2$ cells into a $k$ dimensional real vector, resulting in a $k^3$ dimensional cost $\cost \in \mathbb{R}^n$ where $n=k^3$.
Thus, our objective is to learn the parameters $\theta_\cost$ of the LeNet, along with the constraint matrix $\A$ and vector $\rhs$.

\textbf{Dataset details:} We experiment with $3$ different datasets for $k = 4,6,$ and $9$.
For standard $9 \times 9$ sudokus, we use a standard dataset from a Kaggle Competition \cite{}.
For $k=4$ and $6$, we use the data generation process described in \cite{nandwani&al22}: first sample a masking percentage $p$ uniformly between 30 to 70\%, and then randomly mask $p\%$ of the cells while ensuring that the generated sudoku puzzle has a unique solution. 
For each $k$, We randomly select $10,000$ samples for training and $500$ samples for testing.

For \textbf{visual-sudoku}, to generate the input images, we use the official train and test split of MNIST. 
Digits in our train and test splits are replaced by images in the MNIST train and test sets respectively, avoiding any leakage.  

\textbf{Hyperparameters and training details:} 
For both symbolic and visual sudoku, we train $3$ different Neural ILP models for the three datasets. \\
$\bullet$ \textbf{Number of learnable constraints:}
For $k=4$ and $6$, we keep $m = (n+1)$ as the number of learnable constraints where $n = k^3$ is the number of binary variables.
For $k=9$, we learn $m=(n+1)/2$ equality constraints, which is equivalent to learning $(n+1)$ inequality constraints with parameter tying. This inductive bias enhances the learnability, which becomes crucial for scaling to $9^3 = 729$ dimensional space. \\
$\bullet$ \textbf{Positive and negative margin:}
We set a value of $0.01$ for both positive and negative margins in all the experiments. This is selected by doing a grid search over $\{0.1,0.01,0.5\}$ on the dataset with smallest puzzle size. \\
$\bullet$ \textbf{Temperature annealing:
}: In all our experiments, we start with a temperature $\tau = 1$ and anneal it by a factor of $0.1$ whenever the performance on a small held out set plateaus. \\
$\bullet$ \textbf{Early stopping:} For all our experiments, we early stop the training based on validation set performance, with a timeout of 12 hours for each experiment.\\
$\bullet$ \textbf{Initialization of $\A$ and $\rhs$}:
\ycom{This is becoming messy because we now have to explain over-parameterization}
As described in \citeauthor{paulus&al21}, we also over-parameterize each constraint hyperplane by an additional learnable offset vector $\offset_i$.
This results in the following hyperplane in the base coordinate system: $\arow{i}^T\var + \rhs_i + \offset_i^T\arow{i}/|\arow{i}| \ge 0$.
We experiment with two ways of initializing the constraint hyperplanes and select the one with better performance on dev set. 
The first method is borrowed from \citeauthor{paulus&al21}: each entry of $\arow{i}$ is selected uniformly between $[-0.5,0.5]$, $\rhs_i$ is initilized at $0.2$ and offset $\offset_i$ is initialized such that it lies in the bounded space $[0.25,0.75]^n$. 
In the second method, each entry of $\arow{i}$ and $\offset_i$ is sampled from a standard Normal distribution and $\rhs_i$ is initialized as $0$.
\ycom{TODO: Write the intuition behind the 2nd method: maximally separated hyperplanes;  More aligned with our regularizer loss..It results in sampling of hyperplanes with their normal directions uniformly sampled from unit hyper-sphere. In expectation, such a selection would result in minimum regularizer loss term ($\ilplossfn_{o})$ 
..}
\\
$\bullet$ \textbf{Negative samples:}
We use all the three strategies described in \cref{subsec:negsampling} for generating negatives. 
For $n$ dimensional binary space, we select all the $n$ one hop neighbors, along with equal number of randomly selected 2,3 and 4 hop neighbors, resulting in a total of $4n$ neighbors.

%The later results in sampling of hyperplanes with their normal directions uniformly sampled from unit hyper-sphere. In expectation, such a selection would result in is also aligned with our regularizer loss term ($\ilplossfn_{o})$ 


\textbf{Baselines:}
In addition to CombOptNet, we also compare against Recurrent Relational Networks (RRN) \cite{palm&al18}: a purely neural approach for reasoning based on Graph Neural Networks.
For RRN, we use the same set of hyperparameters as provided in their paper.
For symbolic sudoku, we also experiment with rectifier networks \cite{pan&al20}: a solver-free way of learning only the constraints via a compressed two layer network with rectifier activations in the hidden layer. For learning $m$ constraints, rectifier network requires only $log(m)$ hidden units, thus making it a great candidate for problems like sudoku where one needs to learn a large number of constraints.


\textbf{Results and discussion:}
\Cref{tab:sudoku} compares the performance and training time of our method against the different baselines described above.
We do not add numbers for rectifier networks in the table, because to our surprise it achieves $0\%$ accuracy on all the sizes, despite learning to correctly classify the positives and negatives during training. 
In contrast, \citeauthor{pan&al20} show that a rectifier network improves performance on many structured prediction tasks in NLP.
This is expected, as for structured prediction, violation of a few constraints may not have a huge impact on performance, but for constraint optimization problems, it is crucial to satisfy \emph{all} the constraints, which it fails to do.

\ycom{TODO: Next, we observe that even a purely neural approach achieves very good performance on all three sizes.
%However, this comes at the cost of interpret-ability of the constraints which are implicitly encoded in the network's weights.
Even for 9 x 9 sudokus, our model trains in less than an hour.
In contrast, comboptnet fails to run even a single batch in 12 hours! 
For 4 x 4 sudokus, CombOptNet could barely complete 4 epochs within the given time of 12 hours, resulting in its poor performance.

We observe that the accuracy of the digit classifier is very poor (around 25\%). Still the ILP is able to exploit the desired structure of the output (or exploit the constraints) to correct the mistakes of the classifier.
}

\begin{table}[]
\captionof{table}{\small Board accuracy and training time for different board sizes of sudoku. RRN is a recurrent GNN based neural reasoning model.}
\label{tab:sudoku}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}
\toprule
 & \multicolumn{6}{c}{\textbf{Board Accuracy (In pct)}} & \multicolumn{6}{c}{\textbf{Training Time (in min.)}} \\ \midrule
 & \multicolumn{3}{c}{\textbf{Symbolic}} & \multicolumn{3}{c}{\textbf{Visual}} & \multicolumn{3}{c}{\textbf{Symbolic}} & \multicolumn{3}{c}{\textbf{Visual}} \\
\textbf{Board Size} & \textbf{4 x 4} & \textbf{6 x 6} & \textbf{9 x 9} & \textbf{4 x 4} & \textbf{6 x 6} & \textbf{9 x 9} & \textbf{4 x 4} & \textbf{6 x 6} & \textbf{9 x 9} & \textbf{4 x 4} & \textbf{6 x 6} & \textbf{9 x 9} \\
\textbf{Neural (RRN)} & 100.00 & 99.10 & 91.30 & 99.80 & 97.50 & 71.10 & 100.00 & 99.10 & 91.30 & 99.80 & 97.50 & 71.10 \\
\textbf{CombOptNet} & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 \\
\textbf{Ours} & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 \\ \bottomrule
\end{tabular}
}
\end{table}





==> sections/experiments_yatin.tex <==
\section{Experiments}
\label{sec:experiments}
The goal of our experiments is to evaluate the effectiveness and scalability of our proposed approach compared to SOTA black-box solver based approach, i.e., CombOptNet \cite{paulus&al21}. We also compare with an appropriately designed neural baseline for each of our datasets.  We experiment on 3 datasets: (a) symbolic and visual sudoku~\cite{} (b) random constraints [] (c) key-point matching []. To measure scalability, in each of the domains, we compare performance of each of the algorithms in terms of time taken, as well as accuracy obtained, for a varying problem sizes. All our experiments were run on a V-100 skylake node, with 16 GB of memory. We next describe details of each of these datasets, experimental methodology and our results. 





%\ycom{See tables in \hyperlink{ https://docs.google.com/spreadsheets/d/1HwxaGb-Hb7qBb5nZqXM-2YZGF7_wa-Z6FKWixysw14g/edit?usp=sharing}{this google sheet}
%}

\begin{comment}
The goal of our experiments is to demonstrate that our \emph{solver-free} framework 
for learning 
%parameters of the cost as well as constraints
in a Neural ILP architecture 
scales to much larger problems as compared to solver based approaches.
Specifically, we compare against CombOptNet \cite{paulus&al21}: a recently proposed solver based approach that calls a black-box solver to compute the gradients \wrt\ the cost $\cost$, the constraint matrix $\A$ and vector $\rhs$.
We also compare against a purely neural approach where ever applicable.

To demonstrate scalability, we first experiment on varying sizes of \textit{symbolic and visual sudoku} puzzles. 
The largest puzzle that we consider has $729$ binary variables and $324$ ground truth equality constraints.
We then experiment on two tasks borrowed from \citet{paulus&al21}, \textit{viz.}
\textit{random constraints} and \textit{keypoint matching}.
On them, we achieve performance comparable to CombOptNet, both in terms of accuracy and training time.
We attribute this to the fact that the ILPs in both of these tasks are quite small and hence not a bottleneck during training.
For example, the largest ILP on these domains has 49 binary variables and 14 constraints,  smaller than even the smallest ILP  in the first two tasks ($4 \times 4$ sudoku with $64$ binary variables and $64$ constraints).

\textbf{Fixed cost, learnable constraints:}
Two  of the four tasks, \textit{viz.} symbolic sudoku and random constraints, involve learning of only the constraint matrix $\A$ and vector $\rhs$.
The cost is given as an input to the Neural ILP model $\model_\Theta$ and objective is to learn $\A$ and $\rhs$ such that solving the ILP with learnt $\A$ and $\rhs$ recovers the solution obtained by using the ground truth constraints.

\textbf{Learable cost and learnable constraints:}
In the remaining two tasks, \emph{viz.}, visual sudoku and keypoint matching, the cost $\cost$ is parameterized by a learnable neural network and objective is to learn both the constraints ($\A$ and $\rhs$), as well as the parameters $\theta_\cost$ of the neural network modeling the cost.

\textbf{Computational Resources:}
\ycom{TODO.}
OUrs on shakuntala \ycom{get the exact specs}
CombOptNet on hpc cpu as call to gurobi was  faster 
on cpu. \ycom{@Rishabh: please add specs}.

Next, we present each of the experiments in detail.
\end{comment}


\input{sections/exp_sudoku}
\input{sections/exp_random_constraints}
\input{sections/exp_keypoint_matching}





==> sections/intro_old.tex <==
\section{Introduction}
\label{sec:intro}
%Neural networks are increasingly becoming popular for solving symbolic tasks such as constraint satisfaction problems, playing sudoku, solving combinatorial problems etc. 
Any deployable AI system would most likely involve both perception and reasoning. 
Neural models have achieved state-of-the-art performance in many perceptual tasks and now many models have been developed for reasoning as well.
Combinatorial problems represent one category of reasoning tasks and recently many neural architectures have been proposed to solve them.
For example, \cite{nandwani&al22, palm&al18} design recurrent Graph Neural Networks for solving puzzles like Sudoku, Graph Coloring etc. 
During training, such models learn and implicitly encode in their parameters the unknown constraints of the underlying combinatorial problem.
During inference, a simple forward pass through such networks output the solution of the given input puzzle.

Another alternative for solving a reasoning task is to design a differentiable layer that cast the reasoning task as solving an optimization problem.
Many works focus on defining a differentiable symbolic layer that learns to explicitly represent the constraints in the language of a specific optimization problem such as an Integer Program (IP).  
%Another line of work focuses on defining a differentiable symbolic layer that learns to explicitly represent the constraints in the language of a symbolic algorithm such as an Integer Program (IP).  
In the forward pass, a symbolic layer invokes a blackbox solver, or a specific algorithm, to find the optima of the learnable combinatorial problem. For example, Gurobi\cite{}, or branch and bound, for solving a parameterized Integer Linear Program (ILP). 
Such optimization problems are either non-differentiable or have zero gradient almost everywhere and hence one can't trivially backpropagate through them.

%such symbolic layers during training.
Many works have proposed different ways to  approximate the gradient of a loss \wrt\  the learnable parameters and the input of such symbolic layers. 
For example, \cite{paulus&al21} define gradients w.r.t both the linear constraints as well as the linear cost of an ILP.
\cite{vlastelica&al20} define gradients \wrt\ the linear cost that is optimized over a known discrete space in the forward pass.
\cite{berthet&al20} replace the discrete optimizer with its continuous perturbed version that computes the expected optima by assuming a noise model around the given cost and define the Jacobian matrix of the expected optima \wrt\ the cost. This Jacobian matrix is then multiplied with the gradient of loss \wrt\ the expected optima to get the gradient \wrt\ the cost. 
\cite{niepert&al21} also exploit the perturbation based methods to compute the gradients but propose a different noise model for the perturbations.

Notably, in all of these works, the computation of gradient(or Jacobian) invokes the symbolic solver. This may become a major bottleneck, specially when the constraints are also learnable and the solver needs to solve the combinatorial problem with intermediate (possibly incorrect) constraints.
This poses a practical limitation on such techniques: when the underlying combinatorial problems are big, both in terms of number of constraints and the dimension of the output space, the training process slows down considerably. 
Often the model may not even train in a reasonable amount of time.
As a result, almost all of such works experiment with very small problems. For example, \cite{paulus&al21} experiments with synthetic data in a $16$ dimensional space with maximum $8$ learnable linear constraints; their largest problem size has only $49$ dimensional variables with $14$ constraints (Graph Matching with $7$ keypoints).

In this work, we propose a novel technique to differentiate through the learnable constraints as well as the learnable cost function of an unknown Integer Linear Program (ILP). 
During training, our technique doesn't solve the ILP to compute the gradients.
Intuitively, we cast the learning of linear constraints as learning a polyhedron such that all the given ground truth solutions of the ILP lie within the polyhedron. 
Each hyperplane of the polyhedron can be considered as a binary linear classifier.
To train each binary classifier, we need both negative and positive samples. 
The given ground truth solutions act as positive samples and we propose multiple ways of sampling negative points.
We propose a margin based loss function to train all the binary linear classifiers and find the hyperplanes of the polyhedron simultaneously. 
Specifically, we make the following contributions:
1. \textbf{\ilploss:} A novel differentiable loss function for learning both the constraints and the cost of an Integer Linear Program.
2. \textbf{Solver-free computation of \ilploss:} 
%To compute \ilploss, 
we propose a novel method for solver-free sampling of negative points.
that are required, in addition to the given solutions, to compute \ilploss.
3. Finally, we validate the efficacy of our technique by  learning the linear constraints of sudoku from symbolic as well as visual inputs and their symbolic solutions. Largest puzzle that we consider ($12 \times 12$ sudokus) involve $1728$ binary variables and $576$ ground truth equality ($1152$ inequality) constraints. 
In addition, we deploy solver-free \ilploss\ to learn constraints of all the synthetic as well as real world problems considered in CombOptNet \cite{paulus&al21} and achieve better or similar performance in all the tasks.

\begin{comment}
1. ILP-Loss: We define a novel differentiable loss function for learning the constraints and the cost of an Integer Linear Program that can model many combinatorial problems such as Sudoku, Weighted Set Covering, Matching etc. 
Differentiability of the ILP-Loss makes it possible to use any ILP Solver as the final layer of an end-to-end neuro-symbolic model, \eg, a neural digit classifier followed by an ILP Solver for the task of visual sudoku. \\
2. Solver-free computation of ILP-Loss: 
Computation of ILPLoss requires access to the actual ground truth solutions (positive points) and we propose different ways of generating negative points for training. Notably, such a computation does not require access to the ILP Solver at all during training, making it possible to learn huge number of constraints over very high dimenional space in an end-to-end fashion. \\
3. Our framework can be seen as a generalization of CombOptNet: a recently proposed method to backprop though ILPs. Recently proposed CombOptNet can be s of 
Computation of the ILP-Loss doesn't require solving the ILP, but only require sampling negatives and positive points. As a result, it get rid \\
\end{comment}



==> sections/methods_14thMay.tex <==
\section{Differentiable ILP Loss}

\label{sec:methods}
\begin{comment}
$
\zerovector
\ilpfn
\gtruth
\A
\cost
\rhs
\var
\ilplossfn
$
\ilploss \\
Structure:
1. Notation and task description. Good to keep a running example. Let’s pick visual sudoku. Should we address the issue of label leakage here? 
2. Definition of ilploss:
        1. High level intuition. Casting it as learning many binary classifiers simultaneously. 
        2. \gtruth acts as positive points
        3. Negative sampling
        4. Handling cost 

\end{comment}

\textbf{Notation and task description
}:
Let a combinatorial problem be represented as a solution of an ILP: 
\begin{equation}
\label{eq:ip}
\ilpfn(\A,\rhs,\cost) = \argmin_\var \cost^T\var  \text{\ \ subject to \ \ } \A\var + \rhs \ge \zerovector,  \var \in \mathbb{Z}^n
\end{equation}
Here $\cost \in \mathbb{R}^n$  represents an $n$ dimensional cost vector and the matrix $\A \in \mathbb{R}^{m \times n}$ and $\rhs \in \mathbb{R}^m$ represent $m$ linear constraints defining the feasible region. 
We represent the $i^{th}$ constraint  $\arow{i}^T\var + \rhs_i \ge 0$, as $\constraint{\arow{i}}{\rhs_i}$, where $\arow{i}$ is the $i^{th}$ row of the constraint matrix $\A$ and $\rhs_i$ is the $i^{th}$ element of vector $\rhs$.
The integer constraints $\var \in \mathbb{Z}^n$ make the problem NP hard.

The inputs $\A, \rhs$, and $\cost$ to the function $\ilpfn()$ can either be the output of a neural network, or could be the learnable parameters. 
For example, in visual-sudoku, the cost $\cost$ is parameterised by the 
prediction of a perceptual neural model decoding an input image of a $k \times k$ sudoku puzzle into a score vector for classifying each of the $k^2$ cells into one of the $k$ digits; $\rhs$ and the constraint matrix $\A$  are learnable parameters of the layer solving the ILP in the forward pass.
We call any model that is used to parameterize any of the $\A, \rhs$ or $\cost$ as the backbone model.\\
\textbf{Parameterization of equality constraints:}
Note that our formulation in \cref{eq:ip}
can easily parameterize an equality constraint: $\arow{i}^T\var = \rhs_i$ by adding an additional constraint $\constraint{\arow{i'}}{\rhs_{i'}}$ with tying of parameters as: $\arow{i'} = -\arow{i}$ and $\rhs_i' = -\rhs_i$.
\ycom{Need to write that we add an $\epsilon$ around $\rhs_i$ and $\rhs_{i'}$}

Given ground truth solution $\gtruth$, our goal is to define a differentiable loss function involving  
$\A,\rhs,\cost$, and the ground truth $\gtruth$, which does not require solving the ILP in \cref{eq:ip}.
The derivative of such a loss function \wrt\ $\A,\rhs$ and $\cost$ can be used to directly learn them or train any backbone model that parameterizes them.

\subsection{A solver-free loss}
The main intuition behind our solver-free loss function comes from the observation that each of the $m$ linear constraints defining the feasible region are essentially $m$ linear binary classifiers (hyperplanes in $\mathbb{R}^n$) separating the ground truth  $\gtruth$ from the infeasible region and the linear cost $\cost$ separates it from other feasible samples. 
Here we  use the term linear classifier and hyperplane interchangeably. 
Learning constraints of an ILP is akin to learning $m$ linear hyperplanes.
To do so, one can consider all the given ground truth samples as positive data points for all the $m$ classifiers.
In the absence of explicitly provided negative samples, we propose a couple of strategies for sampling them from $\mathbb{Z}^n$ for each ground truth $\gtruth$. 
We discuss them in detail in \cref{subsec:negsampling}.
For now, let $\negsamples_{\gtruth}$ be the set of all the negative samples generated by all our sampling techniques for a ground truth positive sample $\gtruth$.
Now notice that all classifiers need to positively classify the feasible ground truth samples.
On the other hand, a negative point becomes infeasible even if it violates any one of the $m$ constraints. 
As a result, it would suffice even if any one of the $m$ classifiers correctly classify it as a negative sample.
But while learning, one cannot assign a negative sample to any one classifier as their parameters are being updated.
Instead, we make a soft assignment depending upon the Euclidean distance of the negative sample from the hyperplane. 

\textbf{Learning the cost vector} $\cost$: 
Note that minimizing $\cost^T\var$ in \cref{eq:ip} results in picking $\gtruth$ amongst all the feasible points.
In this sense, the $\cost$ vector is separating $\gtruth$ from rest of the feasible integral points.
To represent this, we add a new $(m+1)^{th}$ constraint with  
$\arow{m+1} = -\cost$ and 
$\rhs_{m+1} = \cost^T\gtruth$:
\begin{equation}
\label{eq:costconstraint}
\cost^T\var \le \cost^T\gtruth 
%\ \ \text{i.e.}  \ \ 
%\arow{m+1} = -\cost
%\ \ \text{and} \ \ 
%\rhs_{m+1} = \cost^T\gtruth
\end{equation}
Note that only $\gtruth$ amongst the feasible integral points satisfy this constraint as no other feasible integral $\var$ can have the cost less than the optimal $\gtruth$. 
We now formally define our \ilploss.

\textbf{Formulating the \ilploss:} 
Let $\dist(\var;\constraint{\arow{i}}{\rhs_i}) = \frac{\arow{i}^T\var + \rhs_i}{|\arow{i}|}$ represent the signed Euclidean distance of a point $\var \in \mathbb{R}^n$ from the hyperplane
corresponding to the constraint $\constraint{\arow{i}}{\rhs_i}$.
%$\arow{i}\var + \rhs_i$. 
We want the signed distance from all the hyperplanes to be positive for the ground truth samples and negative from at least one hyperplane for all the sampled negative points. 
We operationalize this via a margin based loss function:
\begin{equation}
    \label{eq:ilploss}
\begin{split}
    \ilplossfn(\A,\rhs,\cost,\gtruth | \negsamples_{\gtruth})
    = &
    \frac{1}{m+1} \sum\limits_{i=1}^{m+1} \max\{0,\posmargin - \dist(\gtruth;\constraint{\arow{i}}{\rhs_i})\} 
    \ \ + \ \ \\
    & \frac{1}{|\negsamples_{\gtruth}|}
    \sum\limits_{\yneg \in \negsamples_{\gtruth}} \sum\limits_{i=1}^{m+1} 
    \wt{\yneg}{i}\max\{0,\negmargin + \dist(\yneg;\constraint{\arow{i}}{\rhs_i})\} 
\end{split}
\end{equation}

Here, $\posmargin$ and $\negmargin$ are the hyperparameters representing the margins for the positive and the negative points respectively. 
Note that the positive $\gtruth$ is an optimal point of an ILP, and hence most likely will be close to some of the hyperplanes, necessitating the need for separate margins for negative and positive points.
$\wt{\yneg}{i}$ represents the soft assignment of $\yneg$ to the $i^{th}$ constraint $\constraint{\arow{i}}{\rhs_i}$ and is computed by temperature annealed softmax over the negative distances, ensuring that the hyperplane which is most confident to classify it as negative gets the maximum weight.
Note that such a classifier is the one closest to $\yneg$ if it is incorrectly classified by all the hyperplanes and hence lies within the polytope defined by the constraints.
\begin{equation}
\wt{\yneg}{i} = \frac{e^{\left(-d\left(\yneg;\constraint{\arow{i}}{\rhs_i}\right)/\tau\right)}}
{\sum\limits_{j=1}^{m+1} e^{\left(-d\left(\yneg;\constraint{\arow{j}}{\rhs_j}\right)/\tau\right)}}
\end{equation}
In the above equation, the temperature parameter $\tau$ needs to be annealed as the training progresses.
Intuitively, a high temperature initially can be seen as `\emph{exploration}' for the right constraint that will be violated by $\yneg$.
This is important as the constraints are also being learnt and are almost random initially, so a given negative $\yneg$ should not commit to a particular hyperplane.
As the training progresses, we reduce the temperature $\tau$, ensuring that the most confident classifier gets almost all the weight.

\textbf{Orthogonality Loss Regularizer:
}

\begin{equation}
    \sum\limits_{i,j=0; i \ne j}^{m}    \frac{\arow{i}^T\arow{j}}
         {|\arow{i}||\arow{j}|}
\end{equation}

1. Minimizing the above loss requiring $O(m^2)$ dot product computations, is equivalent to minimizing the loss below, which can be computed in $O(m)$.

\begin{equation}
    \left(\sum\limits_{i=0}^{m}
    \frac{\arow{i}}
         {|\arow{i}|}\right)^{2}
\end{equation}

Next, we discuss different ways of sampling the negative points for computing the \ilploss.
%in \cref{eq:ilploss}.

\subsection{Negative Sampling}
\label{subsec:negsampling}
A meaningful computation of \ilploss\ in \cref{eq:ilploss} depends crucially on the negative samples $\negsamples_\gtruth$.
Randomly sampling negatives from $\mathbb{Z}^n$ is one plausible strategy, but it may not be efficient from the learning perspective: any point which is far away from any of the classifiers will easily be classified as negative and will not contribute much to the loss function.
To overcome this, we propose $3$ alternatives: \\
1. \textbf{Integral k-hop neighbours:} In this strategy, we sample the integral neighbours that are at a Hamming Distance of $k$ from $\gtruth$. 
Note that it is possible for a few integral neighbours to  be feasible \wrt\ the $m$ constraints and thus are not true negatives.
But observe that our cost constraint in \cref{eq:costconstraint} will classify it as negative and thus it won't contribute to the overall loss function.
\\
2. \textbf{Project and sample:} 
In this method, we project the ground truth $\gtruth$ on each of the $m$ hyperplanes and then randomly sample a nearest neighbour of the projection, generating a total of $m$ negatives.
Sampling probability in the $j^{th}$ dimension depends on the $j^{th}$ coordinate of the projection: if value of the $j^{th}$ coordinate is $r \notin \mathbb{Z}$, then we sample $\floor{r}$ and $\ceiling{r}$ with probability $\ceiling{r} - r$ and $r - \floor{r}$ respectively. 
\\
3. \textbf{Batch negatives:} Observe that in order to learn the cost vector, we need samples that are feasible \wrt\ the $m$ learnable constraints, but not \wrt\ the cost constraint in \cref{eq:costconstraint}. 
This ensures that the weight $\wt{\yneg}{m+1}$ corresponding to the cost constraint is highest.
But our earlier sampling strategies cannot ensure selection of such feasible points.
To do so, we consider every other ground truth solution in the batch as a potential negative point. 
This proves to be useful, especially when the $m$ constraints determine the rules of the underlying combinatorial problem and are common for all the ground truth samples.


\subsection{Special case of Binary ILPs with learnable costs}

1. Its quite common to have a Binary ILP (BILP) formulation of a combinatorial problem where cost vector is parameterized by a backbone neural network.\\
2. Unconstrained optimization of the objective function $\cost^T\var$ would assign those bits to 1 that have a low corresponding cost, and conversely, will assign those bits to 0 that have a  high cost, and if such an assignment recovers $\gtruth$, then even the unconstrained optimization suffices. \\
3. Viewing it as unconstrained optimization also lead to a probabilistic interpretation of the cost vector: $\cost[i]$ should be inversely proportional to probability of $i^{th}$ bit being equal to 1 (low cost imply high probability of 1). Considering cost as a negative score, we can operationalize this by defining $prob[i] = sigmoid(-\cost[i])$. \\
This motivates a binary cross entropy loss between $prob[i]$  and $\gtruth[i]$. \\


4. Another alternative is to add a loss  proportional to the value of objective function at $\var=\gtruth$, i.e., $\cost^T\gtruth$. 
It would  push the underlying backbone neural network to generate costs such that $\gtruth$ attains the minimum objective value irrespective of the constraints.\\
5. Specifically, we can add $\cost^T\gtruth + (-\cost)^T(\onevector - \gtruth)$. The first term ensures that $\cost[i]$ is low when ground truth $\gtruth[i]$ is $1$ and the second term ensures that $\cost[i]$ is high when $\gtruth[i]$ is $0$.\\
6. Interestingly, the first term is almost equivalent to considering  $\zerovector$ as a negative sample and the second term is equivalent to considering $\onevector$ as a negative sample: whenever active, the negative loss \wrt\ the cost constraint in
\cref{eq:costconstraint} is proportional to $\negmargin + \cost^T(-\yneg+\gtruth)$,
and replacing $\yneg$ by $\zerovector$ and $\onevector$ gives $\cost^T\gtruth$ and $-\cost^T(\onevector - \gtruth)$ respectively. 





==> sections/methods_marked.tex <==
\section{Differentiable ILP Loss}

\label{sec:methods}
\begin{comment}
$
\zerovector
\ilpfn
\gtruth
\A
\cost
\rhs
\var
\ilplossfn
$
\ilploss \\
Structure:
1. Notation and task description. Good to keep a running example. Let’s pick visual sudoku. Should we address the issue of label leakage here? 
2. Definition of ilploss:
        1. High level intuition. Casting it as learning many binary classifiers simultaneously. 
        2. \gtruth acts as positive points
        3. Negative sampling
        4. Handling cost 

\end{comment}

\subsection{Background and task description}
\label{subsec:notation}
\ycom{We are interested in learning how to solve combinatorial problems that can be expressed as an Integer Linear Program (ILP) with equality as well as inequality constraints:}
\begin{equation}
\label{eq:ipwitheq}
\argmin_\var \cost^T\var  \text{\ \ subject to \ \ } \eqmat\var = \eqrhs ; \ \ineqmat\var + \ineqrhs \ge \zerovector ; \ \  \var \in \mathbb{Z}^n
\end{equation}
Here $\cost \in \mathbb{R}^n$  represents an $n$ dimensional cost vector, the matrix $\eqmat \in \mathbb{R}^{m_1 \times n}$ and $\eqrhs \in \mathbb{R}^{m_1}$ represent $m_1$ linear equality constraints, and the matrix $\ineqmat \in \mathbb{R}^{m_2 \times n}$ and $\ineqrhs \in \mathbb{R}^{m_2}$ represent $m_2$ linear inequality constraints, together defining the feasible region.

Without loss of generality, one can replace an  equality constraint $\eqrow{i}^T\var = \eqrhs_i$ by two inequality constraints: $\eqrow{i}^T\var \ge \eqrhs_i$ and
$\eqrow{i}^T\var \le \eqrhs_i$. 
Here $\eqrow{i}$ and $\eqrhs_i$ represent the $i^{th}$ row of the matrix $\eqmat$ and $i^{th}$ element of the vector $\eqrhs$ respectively.
Using this, one can reduce ILP in \cref{eq:ipwitheq} to an equivalent form with just inequality constraints:
\begin{equation}
\label{eq:ip}
\argmin_\var \cost^T\var  \text{\ \ subject to \ \ } \A\var + \rhs \ge \zerovector,  \var \in \mathbb{Z}^n
\end{equation}

Here matrix $\A \in \mathbb{R}^{m \times n}$ is row-wise concatenation of the matrices $\ineqmat, \eqmat$ and $-\eqmat$.
Vector $\rhs \in \mathbb{R}^m$ is a row-wise concatenation of vectors $\ineqrhs, -\eqrhs$ and $\eqrhs$, and
$m=2m_1+m_2$ is the total number of inequality constraints.
We represent the $i^{th}$ constraint  $\arow{i}^T\var + \rhs_i \ge 0$, as $\constraint{\arow{i}}{\rhs_i}$. %where $\arow{i}$ is the $i^{th}$ row of the constraint matrix $\A$ and $\rhs_i$ is the $i^{th}$ element of vector $\rhs$.
The integer constraints $\var \in \mathbb{Z}^n$ make the problem NP hard.

\textbf{Neural ILP Architecture:
}
In a neural ILP architecture, the constraint matrix $\A$, vector $\rhs$, and the cost vector $\cost$ are neural functions $\fnA, \fnrhs,$ and $\fncost$ (of input $\inp$) parameterized by learnable $\Theta = (\theta_\A, \theta_\rhs, \theta_\cost)$, \ie, 
$\A = \fnA(\inp;\theta_\A)$;
$\rhs = \fnrhs(\inp; \theta_\rhs)$;
$\cost = \fncost(\inp; \theta_\cost)$.
This results in a different ILP for each input $\inp$.
For an input $\inp$, the solution given by a neural ILP model, $\model_\Theta(\inp)$, is nothing but the optima of the following paramterized ILP where $\A,\rhs,\cost$ are replaced by corresponding neural functions $\fnA, \fnrhs, \fncost$ evaluated at input $\inp$:
\begin{equation}
    \label{eq:parameterizedilp}
    \model_\Theta(\inp) = \argmin_\var \left(\fncost(\inp; \theta_\cost)\right)^T\var  \text{\ \ subject to \ \ } \fnA(\inp;\theta_\A)\var + \fnrhs(\inp; \theta_\rhs) \ge \zerovector,  \var \in \mathbb{Z}^n
\end{equation}


\textbf{Example of visual-sudoku:} In $k \times k$ visual-sudoku, the input $\inp$ is an image of a sudoku puzzle and $\gtruth \in \{0,1\}^n$ is the corresponding solution,
represented as a $n=k^3$ dimensional binary vector:
the integer in each of the $k^2$ cells is represented by a $k$ dimensional one-hot binary vector.
Function $\fncost(\inp;\theta_\cost)$ parameterizing the cost is nothing but a neural digit classifier that classifies the content of each of the $k^2$ cells into one of the $k$ classes.
The neural functions $\fnA$ and $\fnrhs$ are independent of the input $\inp$ as the constraints are the same for every $k \times k$ sudoku puzzle.
Therefore,
$\fnA(\inp;\theta_\A) = \theta_\A$, and
$\fnrhs(\inp; \theta_\rhs) = \theta_\rhs$, where
$\theta_\A$ is just a learnable matrix of dimension $m \times n$ and $\theta_\rhs$ is a learnable vector of dimension $m$.
%That is, $\A[i,j] = \theta_\A[i,j]$ and $\rhs[i] = \theta_\rhs[i]$.
See \citet{bartlett&al08} for an ILP formulation of $k \times k$ sudoku with $4k^2$ equality constraints in a $n=k^3$ dimensional binary space $\{0,1\}^n$.
%:each of the $k^2$ cells is filled by an integer between $1$ and $k$ represented by a one-hot $k$ dimensional binary vector.

\textbf{Example of symbolic-sudoku:} In the case of symbolic-sudoku, both  the input $\inp$ and the output $\outp$ are $k^3$ dimensional binary vectors. The empty cells in the input are represented by a $k$ dimensional zero vector.
In contrast to visual-sudoku, here the cost vector is an identity function with no parameters: $\fncost(\inp;\theta_\cost) = \inp$.
The only learnable parameters are the  matrix $\theta_\A$ and the vector $\theta_\rhs$.

%We call any model that is used to parameterize any of the $\A, \rhs$ or $\cost$ as the backbone model.\\
\textbf{Learning Task: } Given a training dataset $\traindata = \{(\inp_s,\gtruth_s) \ | \ s \in \{1 \ldots S\}\}$ with $S$ training samples, the task is to learn the parameters $\Theta = (\theta_\A, \theta_\rhs, \theta_\cost)$, such that $\gtruth_s = \model_\Theta(\inp_s)$ for each $s$.
To do so, one needs to define derivatives $\derivative{\ilplossfn}{\A}, \derivative{\ilplossfn}{\rhs},$ and $\derivative{\ilplossfn}{\cost}$  \wrt\ $\A,\rhs,$ and $\cost$ respectively, of an appropriate loss function $\ilplossfn$.
Once such a derivative is defined, one can easily compute derivatives \wrt $\theta_\A, \theta_\rhs,$ and $\theta_\cost$ using the chain rule: 
$\derivative{\ilplossfn}{\theta_\A} = \derivative{\ilplossfn}{\A} \derivative{\fnA(\inp;\theta_\A)}{\theta_\A}$;
$\derivative{\ilplossfn}{\theta_\rhs} = \derivative{\ilplossfn}{\rhs} \derivative{\fnrhs(\inp;\theta_\rhs)}{\theta_\rhs}$; and
$\derivative{\ilplossfn}{\theta_\cost} = \derivative{\ilplossfn}{\cost} \derivative{\fnA(\inp;\theta_\cost)}{\theta_\cost}$.
\ycom{Hence, in the formulation below, we only worry about computing gradients \wrt\ the constraint matrix $\A$, vector $\rhs$, and the cost vector $\cost$.}

The existing approaches, \eg, \cite{paulus&al21}, explicitly 
need access to current model prediction $\model_\Theta(\inp)$ 
%need to compute $\model_\Theta(\inp)$ in every learning iteration to compute the loss and its derivatives. 
This requires solving the ILP in \cref{eq:parameterizedilp}, making the learning process extremely slow.
In contrast, we present a \emph{`solver-free'} framework for computation of an appropriate loss and its derivatives \wrt\ $\A,\rhs,$ and $\cost$.
Our framework does not require solving any ILP while training, thereby making it extremely scalable as compared to existing approaches.
%Given ground truth solution $\gtruth$, our goal is to define a differentiable loss function involving  $\A,\rhs,\cost$, and the ground truth $\gtruth$, which does not require solving the ILP in \cref{eq:ip}. The derivative of such a loss function \wrt\ $\A,\rhs$ and $\cost$ can be used to directly learn them or train any backbone model that parameterizes them.

\subsection{A solver-free framework}

\ycom{
\textbf{Converting constraint optimization to constraint satisfaction:}
Before we provide the intuition for our approach, we first convert the constraint optimization problem in \cref{eq:ip} to an equivalent constraint satisfaction problem by adding an additional `\textit{cost--constraint}' with 
$\arow{m+1} = -\cost$ and 
$\rhs_{m+1} = \cost^T\gtruth$:
\begin{equation}
\label{eq:costconstraint}
\cost^T\var \le \cost^T\gtruth 
\end{equation}
Note that the above cost--constraint separates the solution $\gtruth$ of the original ILP in \cref{eq:ip} from the other feasible integral points. 
This is because $\gtruth$ must achieve the minimum objective value $\cost^T\gtruth$ amongst all the feasible integral points and hence no other feasible integral point $\var$ can obtain objective value less than $\cost^T\gtruth$.
The new constraint $\constraint{\arow{m+1}}{\rhs_{m+1}}$ together with the original $m$ constraints guarantee that $\gtruth$ is the only solution satisfying all of the $(m+1)$ constraints.
This results in the following equivalent linear constraint satisfaction problem:
\begin{equation}
\label{eq:satisfaction}
\argmin_\var \zerovector^T\var  \text{\ \ subject to \ \ } \A\var + \rhs \ge \zerovector \ \ ; \ \ \cost^T\var \le \cost^T\gtruth \ \ ; \ \   \var \in \mathbb{Z}^n
\end{equation}
Note that constructing such an equivalent satisfaction problem requires access to the solution $\gtruth$ of the original ILP in \cref{eq:ip} and that is already available to us for the training data samples.
By rolling up the cost vector $\cost$ into an additional constraint with the help of $\gtruth$, we have converted our original objective of learning both the cost and constraints to just learning of constraints in \cref{eq:satisfaction}.
Next, we provide an intuition behind our framework for doing so.
}

The main intuition behind our solver-free framework comes from the observation that each of the $m$ linear constraints defining the feasible region are essentially $m$ linear binary classifiers (hyperplanes in $\mathbb{R}^n$) separating the ground truth  $\gtruth$ from the infeasible region.
\ycom{The additional cost--constraint in \cref{eq:costconstraint} separates $\gtruth$ from other integral samples feasible \wrt\ the original $m$ constraints.}
Here we  use the term linear classifier and hyperplane interchangeably. 
Learning constraints of an ILP is akin to simultaneously learning $m$ linear binary classifiers separating $\gtruth$ from other infeasible points \ycom{
along with learning a classifier for cost--constraint, separating $\gtruth$ for other feasible integral points.
}
To do so, one needs negative and positive data points for each of the $m+1$ classifiers.
Note here that for a vector $\gtruth$ to lie inside the feasible region, \emph{all} the classifiers need to classify it positively, 
\ycom{and hence it acts as a positive data point for all the $m+1$ binary classifiers.}
\st{and we know that all the given $S$ ground truth samples $\gtruth_s$ in $\traindata$ must be feasible w.r.t. all the $m$ constraints.
Consequently, one can consider all the given ground truth samples as positive data points for all the $m$ binary classifiers.
}
In the absence of explicitly provided negative samples, we propose a couple of strategies for sampling them from $\mathbb{Z}^n$ for each ground truth $\gtruth_s$. 
We discuss them in detail in \cref{subsec:negsampling}.
For now, let $\negsamples_{\gtruth}$ be the set of all the negative samples generated by all our sampling techniques for a ground truth positive sample $\gtruth$.
%Now notice that all classifiers need to positively classify the feasible ground truth samples.
Now notice that in contrast to a positive point which needs to satisfy \underline{\emph{all}} the $m+1$ constraints,  a negative point becomes infeasible even if it violates \underline{\emph{any one}} of the $m+1$ constraints. 
As a result, it would suffice even if any one of the $m+1$ classifiers correctly classify it as a negative sample (see \cref{fig:classifiers}).
But while learning, one cannot assign a negative sample to any one classifier as their parameters are being updated.
Instead, we make a soft assignment depending upon the Euclidean distance of the negative sample from the hyperplane. 
\begin{comment}
\textbf{Learning the cost vector} $\cost$: 
\textbf{Converting constraint optimization into constraint satisfaction
}
Note that minimizing $\cost^T\var$ in \cref{eq:ip} results in picking $\gtruth$ amongst all the feasible points.
In this sense, the $\cost$ vector is separating $\gtruth$ from rest of the feasible integral points.
To represent this, we add a new $(m+1)^{th}$ constraint with  
$\arow{m+1} = -\cost$ and 
$\rhs_{m+1} = \cost^T\gtruth$:
\begin{equation}
\label{eq:costconstraint}
\cost^T\var \le \cost^T\gtruth 
\end{equation}
Note that only $\gtruth$ amongst the feasible integral points satisfy this constraint as no other feasible integral $\var$ can have the cost less than the optimal $\gtruth$. 
%Therefore, for a given $\gtruth_s$, every other $\gtruth_{s'}, s \ne s' \in \{1 \cdots S\}$ acts as a negative sample for training the cost parameters $\theta_\cost$.
\end{comment}
With this intuition, we now formally define our \ilploss.

\textbf{Formulating solver-free \ilploss:} 
Let $\dist(\var;\constraint{\arow{i}}{\rhs_i}) = \frac{\arow{i}^T\var + \rhs_i}{|\arow{i}|}$ represent the signed Euclidean distance of a point $\var \in \mathbb{R}^n$ from the hyperplane
corresponding to the constraint $\constraint{\arow{i}}{\rhs_i}$.
We want the signed distance from all the hyperplanes to be positive for the ground truth samples and negative from at least one hyperplane for all the sampled negative points. 
We operationalize this via a margin based loss function:
\begin{align}
\label{eq:ilploss}
    \ilplossfn(\A,\rhs,\cost,\gtruth | \negsamples_{\gtruth}) \ \ =& \ \
    \lambda_{pos}\ilplossfn_{+} + 
    \lambda_{neg}\ilplossfn_{-} + 
    \lambda_{orth}\ilplossfn_{o} \text{ \ \ where \ \ } \\
    %\label{eq:posloss}
    \ilplossfn_{+} \ \ =& \ \ \frac{1}{m} \sum\limits_{i=1}^{m} 
    \posloss{\gtruth}{\arow{i}}{\rhs_i} \\
    \ilplossfn_{-} \ \ =& \ \  \frac{1}{|\negsamples_{\gtruth}|}
    \sum\limits_{\yneg \in \negsamples_{\gtruth}} \sum\limits_{i=1}^{m+1} 
    \wt{\yneg}{i}
    \negloss{\yneg}{\arow{i}}{\rhs_i} \\
    \ilplossfn_{o} \ \  =&
        \sum\limits_{i,j=1; i \ne j}^{m}    \frac{\arow{i}^T\arow{j}}
         {|\arow{i}||\arow{j}|} 
         \ \ \simeq \ \  
         \left(\sum\limits_{i=1}^{m}
    \frac{\arow{i}}
         {|\arow{i}|}\right)^{2} \\
    \label{eq:softassign}         
    \wt{\yneg}{i} =& \ \  \frac{e^{\left(-\dist\left(\yneg;\constraint{\arow{i}}{\rhs_i}\right)/\tau\right)}}
{\sum\limits_{j=1}^{m+1} e^{\left(-\dist\left(\yneg;\constraint{\arow{j}}{\rhs_j}\right)/\tau\right)}}
\end{align}
We call $\ilplossfn_{+}, \ilplossfn_{-},$ and $\ilplossfn_{o}$ as the positive, negative and orthogonality loss respectively.
The average in $\ilplossfn_{+}$ ensures that a ground truth sample is positively classified by \underline{\textit{all}} the classifiers.
$\posmargin$ and $\negmargin$ are the hyperparameters representing the margins for the positive and the negative points respectively. 
%Note that the positive $\gtruth$ is an optimal point of an ILP, and hence most likely will be close to some of the hyperplanes, necessitating the need for separate margins for negative and positive points.
$\wt{\yneg}{i}$ in $\ilplossfn_{-}$ represents the soft assignment of $\yneg$ to the $i^{th}$ constraint $\constraint{\arow{i}}{\rhs_i}$ and is computed by temperature annealed softmax over the negative distances in \cref{eq:softassign}.
Softmax ensures that the hyperplane which is most confident to classify it as negative gets the maximum weight.
When $\yneg$ lies inside the feasible region, then the most confident classifier is the one closest to $\yneg$.
The temperature parameter $\tau$ needs to be annealed as the training progresses.
Intuitively, a high temperature initially can be seen as `\emph{exploration}' for the right constraint that will be violated by $\yneg$.
This is important as the constraints are also being learnt and are almost random initially, so a given negative $\yneg$ should not commit to a particular hyperplane.
As the training progresses, we reduce the temperature $\tau$, ensuring that the most confident classifier with least signed distance gets almost all the weight. If $\yneg$ is correctly classified as a negative with a margin $\negmargin$ by \emph{any} classifier \ie, $\dist(\yneg; \constraint{\arow{i}}{\rhs_i}) \le -\negmargin$
for some $i$, then the corresponding negative loss,
$\negloss{\yneg}{\arow{i}}{\rhs_i}$, becomes zero, and a low value of $\tau$ ensures that it gets all the weight.

The last term, $\ilplossfn_{o}$ acts as a regularizer and tries to ensure that no two learnt constraints are the same.
This is done by minimizing the cosine similarity between all the pairs of constraints. 

Finally, the weights $\lambda_{pos}, \lambda_{neg},$ and $\lambda_{orth}$ are computed automatically with a multi-loss weighing technique using coefficient of variations as described in \citet{groenendijk&al21}. 
Intuitively, the loss term with maximum variance over the learning iterations, gets most of the weight.

Next, we discuss different ways of sampling the negative points for computing the \ilploss.
%in \cref{eq:ilploss}.

\subsection{Negative Sampling}
\label{subsec:negsampling}
A meaningful computation of \ilploss\ in \cref{eq:ilploss} depends crucially on the negative samples $\negsamples_\gtruth$.
Randomly sampling negatives from $\mathbb{Z}^n$ is one plausible strategy, but it may not be efficient from the learning perspective: any point which is far away from any of the classifiers will easily be classified as negative and will not contribute much to the loss function.
To overcome this, we propose multiple  alternatives: \\
1. \textbf{Integral k-hop neighbours:} To generate negatives, we sample the integral neighbours that are at a Hamming Distance of $k$ from $\gtruth$. 
Note that it is possible for a few integral neighbours to  be feasible \wrt\ the $m$ constraints, but they must have worse cost than the given ground truth $\gtruth$. If not, then such samples contribute towards learning the cost parameters $\theta_\cost$.
\\
2. \textbf{Project and sample:} 
In this method, we project the ground truth $\gtruth$ on each of the $m$ hyperplanes and then randomly sample a neighbour of the projection, generating a total of $m$ negatives.
Sampling probability in the $j^{th}$ dimension depends on the $j^{th}$ coordinate of the projection: if value of the $j^{th}$ coordinate is $r \notin \mathbb{Z}$, then we sample 
$\floor{r}$ and $\ceiling{r}$ with probability $\ceiling{r} - r$ and $r - \floor{r}$ respectively. 
\\
3. \textbf{Batch negatives:} 
In this strategy, we consider every other ground truth $\gtruth_{s'} \ s' \ne s$ in the minibatch as a potential negative sample for $\gtruth_s$. We call it as a `batch--negative'.
This is particularly useful for learning the cost parameters $\theta_\cost$ when the learnable constraints are the same for all the ground truth samples, such as in sudoku.
In such cases, a batch--negative  $\gtruth_{s'}$ being a feasible point of the original ILP formulation, must always satisfy all of the $m$ learnable constraints of the original ILP in \cref{eq:ip}.
\ycom{Hence, the only way for $\gtruth_{s'}$ to be correctly classified as a negative for $\gtruth_{s}$ is by violating the cost constraint in \cref{eq:costconstraint}, \ie, $\cost^T\gtruth_{s'} > \cost^T\gtruth_{s}$
Learning cost parameters $\theta_\cost$ that result in violation of the cost constraint for every batch--negative helps in ensuring that the ground truth $\gtruth_{s}$ indeed has the minimum cost.
}
\begin{comment}
, \ie, $\arow{i}^T\gtruth_{s'} + \rhs_i \ge 0$.
This makes its distance always positive from all the $m$ hyperplanes, contributing positively to $\ilplossfn_{-}$.
The only way to eventually minimize the corresponding negative loss is by ensuring that the batch--negative gets assigned to the cost hyperplane, \ie, $\wt{\gtruth_{s'}}{i}$ is highest for $i = (m+1)$.
This happens when we learn such cost parameters $\theta_\cost$ that ensure that the cost constraint in \cref{eq:costconstraint} is satisfied by a good margin.
\end{comment}

\begin{comment}
\subsection{Special case of Binary ILPs with learnable costs}

1. Its quite common to have a Binary ILP (BILP) formulation of a combinatorial problem where cost vector is parameterized by a backbone neural network.\\
2. Unconstrained optimization of the objective function $\cost^T\var$ would assign those bits to 1 that have a low corresponding cost, and conversely, will assign those bits to 0 that have a  high cost, and if such an assignment recovers $\gtruth$, then even the unconstrained optimization suffices. \\
3. Viewing it as unconstrained optimization also lead to a probabilistic interpretation of the cost vector: $\cost[i]$ should be inversely proportional to probability of $i^{th}$ bit being equal to 1 (low cost imply high probability of 1). Considering cost as a negative score, we can operationalize this by defining $prob[i] = sigmoid(-\cost[i])$. \\
This motivates a binary cross entropy loss between $prob[i]$  and $\gtruth[i]$. \\


4. Another alternative is to add a loss  proportional to the value of objective function at $\var=\gtruth$, i.e., $\cost^T\gtruth$. 
It would  push the underlying backbone neural network to generate costs such that $\gtruth$ attains the minimum objective value irrespective of the constraints.\\
5. Specifically, we can add $\cost^T\gtruth + (-\cost)^T(\onevector - \gtruth)$. The first term ensures that $\cost[i]$ is low when ground truth $\gtruth[i]$ is $1$ and the second term ensures that $\cost[i]$ is high when $\gtruth[i]$ is $0$.\\
6. Interestingly, the first term is almost equivalent to considering  $\zerovector$ as a negative sample and the second term is equivalent to considering $\onevector$ as a negative sample: whenever active, the negative loss \wrt\ the cost constraint in
\cref{eq:costconstraint} is proportional to $\negmargin + \cost^T(-\yneg+\gtruth)$,
and replacing $\yneg$ by $\zerovector$ and $\onevector$ gives $\cost^T\gtruth$ and $-\cost^T(\onevector - \gtruth)$ respectively. 
\end{comment}




==> sections/related_old.tex <==
\section{Related Works}
\label{sec:relatedworks}
There are broadly three ways in which neural models interact with symbolic methods for solving combinatorial problems.

\textbf{Algorithm Configuration:}
In the first category, known as ‘\textit{algorithm configuration}’, neural methods augment a symbolic algorithm by replacing its handcrafted heuristics with a learning based neural model \cite{bengio&al21}. For example, \cite{kruber&al17} use a classifier over features capturing the current state to predict if Dantzing Wolf decomposition should be applied while solving a Mixed Integer Programs (MIP).

\textbf{Neural models for combinatorial problems:}
In the second category,  a neural model such as a Graph Neural Network (GNN) replaces a combinatorial solver altogether and \textit{implicitly} encode the rules or constraints in their weights. For example, \citet{nandwani&al22, nandwani&al21, palm&al18} train a Recurrent Relational Network for learning to solve puzzles like sudoku, graph coloring, futoshiki etc; \citet{dong&al19} propose Neural Logic Machines (NLMs) that learn lifted first order rules and experiment with blocks world, reasoning on family trees etc; 
\citet{selsam&al19, amizadeh&al19a,amizadeh&al19b} train a GNN for solving any CSP when constraints are \textit{explicitly} given in a standard form such as CNF, DNF or Boolean Circuits.

\textbf{Differentiable optimization layers:}
In the third category, a symbolic method is used as a layer or a node in a neuro-symbolic architecture.

\textbf{Continuous Space:}
\cite{gould&al19} call any node that solves an optimizatation problem in the forward pass as a '\textit{declarative node}' and show how to differentiate through continuous constrained optimization problem. Similar to this are other works \cite{amos&kolter17, agrawal&al19} that define methods for differentiating through other continuous problems like convex quadratic programs (QPs) or cone programs. 
Related is the area of Inverse Optimization \cite{chan&al21} within Operations Research that aims to learn the constraints and/or costs of a linear program from the observed optimal decisions.
Recently \cite{tan&al19, tan&al20} use the notion of Parameterised Linear Programs (PLP) in which both the cost and the constraints of an LP are parameterised by unknown weights and a feature vector. 
They apply deep learning techniques for learning the parameters given pairs of features and optimal decisions. Specifically, \citet{tan&al19} differentiate through the unrolled steps of log-barrier interior point method for constrained optimisation and \citet{tan&al20} pose Inverse Optimization itself as a bi-level constrained optimization problem, minimizing an appropriate loss between the current solution and observed solution subject to the feasibility of the observed solution and optimality of the current solution w.r.t. the current parameters. 


\textbf{Discrete space:}
\textbf{Using a specific algorithm/ relaxation:}
For the case of discrete problems, some works focus on a specific symbolic algorithm or its approximation and define how to differentiate through them. For example, \citet{wang&al19} uses a low rank SDP relaxation of MAXSAT and defines how the gradients flow during backpropagation;
\citet{ferber&al20} backprop through the KKT conditions of the LP relaxation created iteratively while using cutting-plane method \cite{gomory10} for solving a MILP;
\citet{wilder&al19} add a quadratic penalty term to the continuous relaxation and use implicit function theorem to backprop through the KKT conditions, as done in \citet{amos&kolter17} for smooth programs;
\citet{mandi&guns20} instead add a log-barrier term to get the LP relaxation and instead of differentiating through its KKT conditions, they differentiate through its homogeneous self-dual formulation and link it to the iterative steps in the interior point method.

\textbf{Discrete space: Black-box solver:}
\textbf{Known constraints:}
Instead of working with a specific algorithm, many works differentiate through a black-box combinatorial solver.
\cite{vlastelica&al20} define gradient w.r.t. linear cost function that is optimized over a given discrete space. \cite{rolinek&al20a, rolinek&al20b}
exploit it for the task of Deep Graph Matching, and for differentiating through rank based metrics such as Average Precision/Recall respectively.
\cite{berthet&al20} replace the black-box discrete solver with its smooth perturbed version during training and exploit 'perturb-and-MAP' \cite{papandreou&yuille11} to compute the gradients.
On similar lines, \cite{niepert&al21} also exploit perturb-and-MAP but propose a different noise model for perturbation and also extends to the case when the output of the solver may feed into a downstream neural model.

The above works differentiating through the black-box solvers assume that the constraints of the discrete optimization problem are known apriori and one needs to differentiate only through the linear cost function.

\textbf{Discrete space: Black-box solver:}
\textbf{Unknown constraints:}
Extending it further, \cite{paulus&al21} aims to learn the linear constraints along with the cost function of an ILP.
\ycom{write a line about them}
%They define a smooth approximation of the function that maps any cost vector to the corresponding optima and define the gradients of the linear cost and constraints using the gradient of the loss w.r.t. the optima.
However, a major drawback of all the methods differentiating through black-box solvers is that they need to call the solver for computing the gradients. 
This becomes a bottleneck especially during the training when the constraints are also being learnt and hence the overall problem could be ill-defined. 
In this work, we propose a loss function whose computation does not require calling the solver.
We treat each constraint of the ILP as a parameterized linear classifier whose weights need to be learnt. For training, the given outputs act as positive points for all the classifiers and we use multiple methods for sampling negative points, including our novel project-and-round sampling technique that first projects each positive on each of the hyperplane and then round the projection to find an integral negative sample.
Closely related to our idea is \cite{pan&al20} for structured prediction that also aims to learn the linear constraints over the output variables but compactly represent them using a specific two layer Rectifier Network \cite{pan&srikumar16}. 
A major difference is that their method cannot be used for simultaneously learning the cost and the constraints.
\cite{meng&chang21} propose a non-learning based approach for mining constraints in which for each training data $(c,y)$, a new constraint is added which essentially imply that no other target can have better cost than the given target $y$ for the corresponding cost $c$.  



\ycom{check how to place smart predict then optimise \cite{elmachtoub&grigas22}.
There is something called task based loss functions which are computed between the output of optimization method and the given gold target. Smart predict then optimise and \cite{donti&al17} falls under this category. Not sure how to place it in the current taxonomy.
}

\ycom{Also need to cite polytope learning paper}

